A Spectral Method for Joint Community Detection and Orthogonal Group Synchronization

Community detection and orthogonal group synchronization are both fundamental problems with a variety of important applications in science and engineering. In this work, we consider the joint problem of community detection and orthogonal group synchronization which aims to recover the communities and perform synchronization simultaneously. To this end, we propose a simple algorithm that consists of a spectral decomposition step followed by a blockwise column pivoted QR factorization (CPQR). The proposed algorithm is efficient and scales linearly with the number of edges in the graph. We also leverage the recently developed `leave-one-out' technique to establish a near-optimal guarantee for exact recovery of the cluster memberships and stable recovery of the orthogonal transforms. Numerical experiments demonstrate the efficiency and efficacy of our algorithm and confirm our theoretical characterization of it.

==> textfile/preliminary.tex <==
\section{Preliminary}
\label{sec:pre}

First, we introduce an operator that measures the ``angle" between two subspaces in the following which is frequently used in our analysis:
\begin{definition}
For any matrix $\bm{X} \in \mathbb{R}^{m \times n}$, let $\bm{X} = \bm{U}\bm{\Sigma}\bm{V}^{\top}$ be the singular value decomposition of $\bm{X}$, then we define a matrix operator $P(\cdot)$ as
\begin{equation*}
    P(\bm{X}) = \bm{U}\bm{V}^{\top}.
\end{equation*}
\end{definition}
The main purpose of introducing $P(\cdot)$ is to appropriately measure the distance between two subspaces. To do this, let $\bm{X}$ and $\bm{Y}$ be two matrices of the same size whose columns are orthogonal and span two subspaces. Clearly, $\|\bm{X} - \bm{Y}\|_2$ is not a proper metric of the distance since it does not account the global orthogonal transformation on the columns of $\bm{X}$ and $\bm{Y}$. Therefore, we define
\begin{equation}
    \text{dist}(\bm{X}, \bm{Y}) = \min_{\bm{Q} \in \mathrm{O}(d)} \|\bm{X} - \bm{Y}\bm{Q}\|_2
    \label{eq:dist_subspace}
\end{equation}
to be the distance which is invariant to any global rotation. Also, the explicit form of $\bm{Q}^*$ that minimize $\|\bm{X} - \bm{Y}\bm{Q}\|_2$ can be easily derived as 
\begin{equation*}
    \bm{Q}^* = P(\bm{Y}^\top\bm{X}).
\end{equation*}
The metric defined in Eq.~\eqref{eq:dist_subspace} will be frequently used in our analysis. 

The following result provides an upper bound of $\|P(\bm{X}) - P(\bm{Y})\|_2$, when both matrices $\bm{X}$ and $\bm{Y}$ are square and invertible:
\begin{lemma}{\textup{\cite[Lemma 5.2]{ling2020near}}}
For two $d \times d$ invertible matrices $\bm{X}$ and $\bm{Y}$, it holds that 
\begin{equation*}
    \|P(\bm{X}) - P(\bm{Y})\|_2 \leq 2\sqrt{2}\min\{\sigma^{-1}_{\text{min}}(\bm{X}), \sigma^{-1}_{\text{min}}(\bm{Y})\}\|\bm{X} - \bm{Y}\|_2,
\end{equation*}
where $\sigma_{\text{min}}(\cdot)$ denotes the smallest singular value of a matrix.
\label{lemma:PX_PY}
\end{lemma}

The following classical result characterizes the property of singular values, eigenvalues and eigenvectors when a matrix is perturbed by a certain amount. 
\begin{theorem}[Weyl's inequality~\cite{stewart1998perturbation}]
Let $\bm{X}$ and $\bm{Y}$ be two matrices of the same size, it satisfies
\begin{equation*}
    |\sigma_i(\bm{X}) - \sigma_i(\bm{Y})| \leq \|\bm{X} - \bm{Y}\|_2, \; \forall i 
\end{equation*}
where $\sigma_i(\cdot)$ denotes the $i$-th largest singular value of a matrix.
\label{the:weyl}
\end{theorem}

\begin{theorem}[Davis-Kahan $\sin(\theta)$ theorem~\cite{davis1970rotation}]
Let $\bm{X} \in \mathbb{R}^{n\times n}$ and $\hat{\bm{X}} = \bm{X} + \bm{\Delta} \in \mathbb{R}^{n\times n}$ be two symmetric matrices with eigenvalues $\{\lambda_i\}_{i = 1}^n$ and $\{\hat{\lambda}_i\}_{i = 1}^n$ respectively.
Then $\bm{X}$ and $\hat{\bm{X}}$ satisfy the following eigen-decompositions:
\begin{equation*}
    \bm{X} = 
    \begin{bmatrix}
    \bm{\Phi}_0 &\bm{\Phi}_1
    \end{bmatrix}
    \begin{bmatrix}
    \bm{\Lambda}_0 &\bm{0}\\
    \bm{0} &\bm{\Lambda}_1
    \end{bmatrix}
    \begin{bmatrix}
    \bm{\Phi}_0 &\bm{\Phi}_1
    \end{bmatrix}^\top, \quad
    \hat{\bm{X}} = 
    \begin{bmatrix}
    \hat{\bm{\Phi}}_0 &\hat{\bm{\Phi}}_1
    \end{bmatrix}
    \begin{bmatrix}
    \hat{\bm{\Lambda}}_0 &\bm{0}\\
    \bm{0} &\hat{\bm{\Lambda}}_1
    \end{bmatrix}
    \begin{bmatrix}
    \hat{\bm{\Phi}}_0 &\hat{\bm{\Phi}}_1
    \end{bmatrix}^\top
\end{equation*}
where $\bm{\Lambda}_0$ (resp. $\hat{\bm{\Lambda}}_0$) is the diagonal matrix that contains the top $d$ eigenvalues $\{\lambda_i\}_{i = 1}^d$ of $\bm{X}$ (resp.  $\{\hat{\lambda}_i\}_{i = 1}^d$ of $\hat{\bm{X}}$), and $\bm{\Lambda}_1$ (resp. $\hat{\bm{\Lambda}}_1$) is the diagonal matrix with the remaining eigenvalues, the columns of $\bm{\Phi}_k$ and $\hat{\bm{\Phi}}_k$ are the corresponding eigenvectors. Then it satisfies
\begin{equation*}
    \left\|\hat{\bm{\Phi}}_1^\top\bm{\Phi}_0\right\|_2 \leq \frac{\|\bm{\Delta}\bm{\Phi}_0\|_2}{\delta}
\end{equation*}
where $\delta$ denotes the spectral gap between $\hat{\bm{\Lambda}}_0$ and $\bm{\Lambda}_1$, i.e. $\delta = |\lambda_{\text{min}}(\hat{\bm{\Lambda}}_0) - \lambda_{\text{max}}(\bm{\Lambda}_1)|$.
\label{the:davis_kahan}
\end{theorem}

Theorem~\ref{the:davis_kahan} defines another metric of the distance between two subspaces as $\text{dist}(\bm{\Phi}_0,\; \hat{\bm{\Phi}}_0) =  \left\|\hat{\bm{\Phi}}_1^\top\bm{\Phi}_0\right\|_2$, where $\hat{\bm{\Phi}}_1$ is the complement subspace of $\hat{\bm{\Phi}}_0$. However, in our analysis we are more interested in measuring the difference $\|\bm{\Phi}_0 - \hat{\bm{\Phi}}_0\bm{O}\|$ defined in Eq.~\eqref{eq:dist_subspace}. Therefore, the following result establishes the connection between these two measurements:

\begin{lemma}[\textup{\cite[Lemma 5.6]{ling2020near}}]
Suppose $\bm{X}_0 \in \mathbb{R}^{n \times d}$ and $\bm{Y}_0 \in \mathbb{R}^{n \times d}$ are two matrices of the same size with orthogonal columns, i.e. $\bm{X}_0^\top\bm{X}_0 = \bm{Y}_0^\top\bm{Y}_0 = \bm{I}_d$, let $\bm{X}_1$ and $\bm{Y}_1$ be the complement subspace of $\bm{X}_0$ and $\bm{Y}_0$ respectively. Then it satisfies
\begin{equation*}
    \left\|\bm{Y}_0 - \bm{X}_0\bm{O}\right\|_2 \leq 2\left\|\bm{X}_1\bm{Y}_0\right\|_2,
\end{equation*}
where $\bm{O} = P(\bm{X}_0^\top\bm{Y}_0)$.
\label{lemma:error2inner}
\end{lemma}
